Spectral sequences from $\mathrm{St}$ homology recovering $J^-$ and $J^+$

Arnold's invariants are $\mathrm{St}$, $J^-$, and $J^+=J^-+\text{the number of double points}$. The quantization polynomials of $\mathrm{St}$ include the vertex state sum $\mathrm{St}_q^v$ (2023, doi:10.1142/S0129167X23500672) and the edge state sum $\mathrm{St}_q$ (arXiv:2610.36387v1). The edge state sum is used for categorification. The quantization polynomial $P_C(q)$ of $J^-$ is due to Viro (1996, "Generic immersions of the circle to surfaces and the complex topology of real algebraic curves"). By the relation $J^+=J^-+\text{the number of double points}$, the quantization polynomial of $J^+$ is obtained, in essence, from $P_C(q)$ together with the quantization polynomial $V_q$ of the number of double points (Lanzat and Polyak, Topology Appl. 160 (2013), 871-874). These categorifications were obtained in arXiv:2610.36387v1 and arXiv:2609.11427v1. We call the homological lifts of $\mathrm{St}_q$, $P_C(q)$, and $V_q$ St homology, $J^-$ homology, and double-point-count $V$ homology, respectively. The pair of the latter two, which gives the homological lift of $J^+$, is called $J^+$ homology. The main result can then be stated as follows. Using de Rham and Koszul complexes, we construct two spectral sequences of families of complexes containing St homology, converging to $J^-$ homology and to the image of the coefficient sequences obtained from double-point-count $V$ homology, respectively, and obtain $J^+$ homology. The spectral sequences thus directly relate the homological lifts of the quantization polynomials of Arnold's three invariants.

==> FromStToJ_figure_geometry.tex <==
% Input inside a local group. The flow arrows and contour arrows are distinct.
\tikzset{
  fromsttoj contour/.style={line width=.66pt, line cap=round, line join=round},
  fromsttoj flow/.style={-{Stealth[length=5pt,width=4pt]}},
  fromsttoj orientation/.style args={#1}{
    postaction={decorate},
    decoration={markings,mark=at position #1 with {\arrow{To[length=2.8pt,width=3.5pt]}}}
  },
  fromsttoj three orientations/.style={
    postaction={decorate},
    decoration={markings,
      mark=at position .17 with {\arrow{To[length=2.8pt,width=3.5pt]}},
      mark=at position .47 with {\arrow{To[length=2.8pt,width=3.5pt]}},
      mark=at position .78 with {\arrow{To[length=2.8pt,width=3.5pt]}}
    }
  }
}

\newcommand{\FromStToJBasedCurve}[1]{%
  \draw[#1] (-1.34,.62) -- (1.05,.62)
    .. controls (1.62,.65) and (1.40,.92) .. (1.22,1.05)
    .. controls (1.02,1.25) and (.74,.85) .. (.57,.62)
    .. controls (.35,.32) and (.13,.17) .. (0,.01)
    .. controls (-.24,-.28) and (-.60,-.72) .. (-.38,-.72)
    .. controls (.13,-.76) and (.50,-.62) .. (.33,-.36)
    .. controls (.24,-.22) and (.12,-.16) .. (0,.01)
    .. controls (-.18,.25) and (-.30,.44) .. (-.52,.62)
    .. controls (-.74,.87) and (-.96,1.15) .. (-1.12,1.10)
    .. controls (-1.34,1.01) and (-1.64,.64) .. (-1.34,.62) -- cycle;
  \fill (-1.34,.62) circle[radius=1.3pt];
}

\newcommand{\FromStToJLeftCircle}{%
  (-.385,.34)
    .. controls (-.305,.46) and (-.397,.70) .. (-.529,.702)
    .. controls (-.700,.71) and (-.777,.565) .. (-.747,.43)
    .. controls (-.727,.317) and (-.561,.258) .. cycle
}
\newcommand{\FromStToJRightCircle}{%
  (.374,.334)
    .. controls (.501,.282) and (.653,.343) .. (.686,.465)
    .. controls (.707,.591) and (.626,.711) .. (.506,.698)
    .. controls (.387,.687) and (.314,.470) .. cycle
}
\newcommand{\FromStToJBottomCircle}{%
  (-.020,-.563)
    .. controls (-.144,-.551) and (-.210,-.668) .. (-.183,-.761)
    .. controls (-.164,-.870) and (-.021,-.929) .. (.075,-.874)
    .. controls (.193,-.802) and (.169,-.588) .. cycle
}
\newcommand{\FromStToJMiddleTop}{%
  .. controls (-.132,.272) and (.105,.270) .. (.230,.245)
}
\newcommand{\FromStToJMiddleRight}{%
  .. controls (.298,.226) and (.189,.007) .. (.128,-.130)
  .. controls (.088,-.218) and (.037,-.355) .. (-.011,-.385)
}
\newcommand{\FromStToJMiddleLeft}[1]{%
  .. controls (-.101,-.393) and (-.204,-.209) .. (-.233,-.128)
  .. controls (-.298,.056) and (-.290,.206) .. #1
}

\newcommand{\FromStToJCircleConfiguration}[4]{%
  \draw[#1] \FromStToJLeftCircle;
  \draw[#2] (-.234,.245) \FromStToJMiddleTop
    \FromStToJMiddleRight \FromStToJMiddleLeft{cycle};
  \draw[#3] \FromStToJRightCircle;
  \draw[#4] \FromStToJBottomCircle;
}

\newcommand{\FromStToJMarkedPoints}{%
  \foreach \point in {(-.385,.34),(-.234,.245),(.230,.245),
                     (.374,.334),(-.011,-.385),(-.020,-.563)} {
    \fill \point circle[radius=1.18pt];
  }%
}

\newcommand{\FromStToJStState}{%
  % At the left crossing, both circles enter one end of the wide edge
  % and leave the other. The two remaining crossings have dotted markers.
  \draw[fromsttoj orientation=.15] (-.329,.384)
    .. controls (-.322,.529) and (-.396,.708) .. (-.529,.702)
    .. controls (-.700,.71) and (-.794,.565) .. (-.759,.423)
    .. controls (-.736,.304) and (-.564,.309) .. (-.436,.236);
  \draw[fromsttoj three orientations] (-.272,.342)
    .. controls (-.159,.310) and (.098,.301) .. (.230,.245)
    \FromStToJMiddleRight
    .. controls (-.101,-.393) and (-.214,-.215) .. (-.258,-.116)
    .. controls (-.312,.008) and (-.350,.125) .. (-.379,.194);
  \draw (-.436,.236) -- (-.329,.384) (-.379,.194) -- (-.272,.342);
  \draw (-.436,.236) -- (-.379,.194) (-.329,.384) -- (-.272,.342);
  \draw[fromsttoj orientation=.18] \FromStToJRightCircle;
  \draw[fromsttoj orientation=.17] \FromStToJBottomCircle;
  \draw[densely dotted] (.230,.245) -- (.374,.334)
    (-.011,-.385) -- (-.020,-.563);
}

